A Toolchain for Streaming Dataflow Accelerator Designs for Big Data Analytics: Defining an IR for Composable Typed Streaming Dataflow Designs

Tydi is an open specification for streaming dataflow designs in digital circuits, allowing designers to express how composite and variable-length data structures are transferred over streams using clear, data-centric types. This provides a higher-level method for defining interfaces between components as opposed to existing bit- and byte-based interface specifications. In this thesis, an open-source intermediate representation (IR) is introduced which allows for the declaration of Tydi's types. The IR enables creating and connecting components with Tydi Streams as interfaces, called Streamlets. It also lets backends for synthesis and simulation retain high-level information, such as documentation. Types and Streamlets can be easily reused between multiple projects, and Tydi's streams and type hierarchy can be used to define interface contracts, which aid collaboration when designing a larger system. The IR codifies the rules and properties established in the Tydi specification and serves to complement computation-oriented hardware design tools with a data-centric view on interfaces. To support different backends and targets, the IR is focused on expressing interfaces, and complements behavior described by hardware description languages and other IRs. Additionally, a testing syntax for the verification of inputs and outputs against abstract streams of data, and for substituting interdependent components, is presented which allows for the specification of behavior. To demonstrate this IR, a grammar, parser, and query system have been created, and paired with a backend targeting VHDL.

==> body/background/interfaces.tex <==
\section{Interface Specifications}\label{sec:background_interfaces}

\todo{Likewise, interfaces can be a background section}

% While improved languages and frameworks can speed up design and improve reusability \cite{izraelevitzreusability2017}, interface standards such as \cite{armlimitedamba2010, armlimitedintroduction2021, intelcorporationavalon2022, pontesscaffi2007} ensure that IPs can be made compatible between projects. Additionally, design tools provide catalogs of IPs and methods to combine and integrate them into larger designs \cite{advancedmicrodevicesinc.intellectual2022, intelcorporationintroduction2021}.

\todo{AXI4(-Stream)}

\todo{Avalon}

\todo{Scaffi}

==> preface.tex <==
\chapter*{Preface}
\setheader{Preface}

Preface\ldots

\begin{flushright}
{\makeatletter\itshape
    \@author \\
    Delft, July 2022
\makeatother}
\end{flushright}



==> sum/2_introduction/motivation.tex <==
\section{Motivation}\label{sec:motivation}

\todo{Motivation (currently copied from paper)}

While much research is focused on developing and accelerating algorithms for streaming data in both hardware \cite{nowatzkistreamdataflow2017, plavecstream2010} and software \cite{isahsurvey2019}, many designs for low-level hardware still have to transfer streams over interfaces which are either custom or based on generic, bit- and/or byte-oriented specifications such as AXI4-Stream \cite{armlimitedamba2010} and Avalon-ST \cite{intelcorporationavalon2022}. As a result, higher-level information about data structures and how streams of data are organized over transfers must be devised and implemented by designers, and are not reflected by the declaration of the interface in a traditional HDL.

Some of this design effort can be alleviated through the use of high-level synthesis: tools such as Vivado HLS can be employed to leverage C, C++ or SystemC combined with IP-blocks using \textit{ap\_fifo} or AXI4-Stream to handle data streams \cite{advancedmicrodevicesinc.interfaces2022}, while synthesizing compilers such as Optimus \cite{hormatioptimus2008} have been developed in the past to leverage StreamIt \cite{thiesstreamit2002}, a language specifically for streaming applications. At the same time, many researchers are working on improved hardware description languages and IRs, such as Chisel \cite{bachrachchisel2012}, FIRRTL \cite{izraelevitzreusability2017} and LLHD \cite{schuikillhd2020}.

These are not suitable replacements for a higher-level interface specification, however: HLS tools either obfuscate the interfaces between low-level hardware and/or use proprietary IRs and tools to connect components, making reuse more difficult. While the HDLs and IRs mentioned are aimed at more general hardware designs, so still require custom interfaces for streaming data transfers. As such, we propose a free, open-source IR for defining high-level streaming dataflow interfaces mapped onto hardware and for connecting these interfaces. This complements existing HDLs and IRs which describe behavior, and enabling components designed in higher-level front-end languages for HLS to propagate more type information to the resulting interfaces.

\todo{Expand on how we want a full toolchain...}



Working towards a full toolchain, there is a separate project for a front-end and language for expressing behavior, called Tydi-lang.

==> tables/complexity_levels.tex <==
\scriptsize
    \centering
    \begin{tabulary}{\linewidth}{L|L|L|L}
\textbf{Complexity} & \textbf{Dimension Information} & \textbf{Sequence Transfer Requirements}                                                                                                  & \textbf{Notes}                                                                                                                                                                                   \\ \hline
1                   & Per transfer, on active data   & Entire sequence must be   transferred in consecutive lanes, with all possible lanes active, over   consecutive cycles.                   & Uses endi (end index) to pad the   end of a sequence when using multiple element lanes. (E.g., when fitting a   sequence of 2 elements in 3 element lanes.)                                      \\ \hline
2                   & Per transfer, on active data   & Innermost sequences (dimension   0) must be transferred in consecutive lanes, with all possible lanes active,   over consecutive cycles. & May set valid = '0' after an   innermost sequence                                                                                                                                                \\ \hline
3                   & Per transfer, on active data   & Innermost sequences (dimension   0) must be transferred in consecutive lanes, with all possible lanes active.                            & May set valid = '0' after any   transfer                                                                                                                                                         \\ \hline
4                   & \textit{Per transfer}          & Innermost sequences (dimension   0) must be transferred in consecutive lanes, with all possible lanes active.                            & May use strb = '0' with valid =   '1' to transfer dimension information after a transfer with active data.                                                                                       \\ \hline
5                   & Per transfer                   & Innermost sequences (dimension   0) must be transferred in consecutive lanes, aligned to lane 0.                                         & Does not need to fill all   element lanes until done transferring an innermost sequence. (May split an   innermost sequence of 2 elements over 2 transfers, even when 2+ lanes are   available.) \\ \hline
6                   & Per transfer                   & Innermost sequences (dimension   0) must be transferred in consecutive lanes.                                                            & Can use stai (start index) to   set the starting lane.                                                                                                                                           \\ \hline
7                   & Per transfer                   & None                                                                                                                                     & Can use strb (strobe) to set   individual lanes inactive.                                                                                                                                        \\ \hline
8                   & \textit{Per element}           & None                                                                                                                                     & Has a last signal per element   lane.                                                                                                                                                           
\end{tabulary}
